Theoretical Guarantees for Variational Inference with Fixed-Variance Mixture of Gaussians

Variational inference (VI) is a popular approach in Bayesian inference, that looks for the best approximation of the posterior distribution within a parametric family, minimizing a loss that is typically the (reverse) Kullback-Leibler (KL) divergence. Despite its empirical success, the theoretical properties of VI have only received attention recently, and mostly when the parametric family is the one of Gaussians. This work aims to contribute to the theoretical study of VI in the non-Gaussian case by investigating the setting of Mixture of Gaussians with fixed covariance and constant weights. In this view, VI over this specific family can be casted as the minimization of a Mollified relative entropy, i.e. the KL between the convolution (with respect to a Gaussian kernel) of an atomic measure supported on Diracs, and the target distribution. The support of the atomic measure corresponds to the localization of the Gaussian components. Hence, solving variational inference becomes equivalent to optimizing the positions of the Diracs (the particles), which can be done through gradient descent and takes the form of an interacting particle system. We study two sources of error of variational inference in this context when optimizing the mollified relative entropy. The first one is an optimization result, that is a descent lemma establishing that the algorithm decreases the objective at each iteration. The second one is an approximation error, that upper bounds the objective between an optimal finite mixture and the target distribution.

==> background.tex <==

\subsection{Wasserstein geometry}\label{sec:wasserstein_geometry}

For two given probability distributions $\nu$ and $\mu$ in $\mathcal{P}_2(\X)$, we denote by $\Pi(\nu,\mu)$ the set of possible couplings between $\nu$ and $\mu$. In other words $\Pi(\nu,\mu)$ contains all possible distributions $\pi$ on $\X\times \X$ such that if $(X,Y) \sim \pi $ then $X \sim \nu $ and $Y\sim \mu$. The $2$-Wasserstein distance on $\mathcal{P}_2(\X)$ is defined by means of an optimal coupling between $\nu$ and $\mu$ in the following way:
\begin{align}\label{eq:wasserstein_2}
W_2^2(\nu,\mu) := \inf_{\pi\in\Pi(\nu,\mu)} \int \left\Vert x - y\right\Vert^2 \dd \pi(x,y) \qquad \forall \nu, \mu\in \mathcal{P}_2(\X).
\end{align}
It is a well established fact that such optimal coupling $\pi^*$ exists \cite{villani2009optimal}. %\ak{as soon as the ambiant space X, here Rd is convex} 
Moreover, it can be used to define a path $(\rho_t)_{t\in [0,1]}$ between $\nu$ and $\mu$ in $\mathcal{P}_2(\X)$. For a given time $t$ in $[0,1]$ and given a sample $(x,y)$ from $\pi^{*}$, it is possible to construct a sample $z_t$ from $\rho_t$ by taking the convex combination of $x$ and $y$: $z_t = s_t(x,y)$ where $s_t$ is given by:
\begin{equation}\label{eq:convex_combination}
s_t(x,y) = (1-t)x+ty \qquad \forall x,y\in \X, \; \forall t\in [0,1].
\end{equation}
The function $s_t$ is well defined since $\X$ is a convex set. More formally, $\rho_t$ can be written as the projection or push-forward of the optimal coupling $\pi^{*}$ by $s_t$:  
\begin{equation}\label{eq:displacement_geodesic}
\rho_t = (s_t)_{\#}\pi^{*}
\end{equation}
We recall that for any measurable map $T: \X \rightarrow \X$ and any $\rho \in \mathcal{P}(\X)$, the push-forward measure $T_{\#}\rho$ is characterized by the following transfer lemma:
\begin{align}
\int_{y \in \X} \phi(y) \dd T_{\#}\rho(y) =\int_{x \in \X}\phi(T(x)) \dd \rho(x) \text{ for every measurable and bounded function $\phi$.}
\end{align}
It is easy to see that \Cref{eq:displacement_geodesic} satisfies the following boundary conditions at $t=0,1$:
\begin{align}\label{eq:boundary_conditions}
\rho_0 = \nu \qquad \rho_1 = \mu.
\end{align}
Paths of the form of \Cref{eq:displacement_geodesic} are called \textit{displacement geodesics}. They can be seen as the shortest paths from $\nu$ to $\mu$ in terms of mass transport (\cite{santambrogio2015optimal} Theorem 5.27). It can be shown that there exists a \textit{velocity vector field} $(t,x)\mapsto v_t(x)$ with values in $\R^d$ such that $\rho_t$ satisfies the continuity equation:
\begin{equation}\label{eq:continuity_equation}
  \frac{\partial \rho_t}{\partial t} + \div(\rho_t v_t ) = 0 \qquad \forall t\in[0,1].
\end{equation}
This equation expresses two facts, the first one is that $-div(\rho_t v_t)$ reflects the infinitesimal changes in $\rho_t$ as dictated by the vector field  $v_t$, the second one is that the total mass of $\rho_t$ does not vary in time as a consequence of the divergence theorem. \Cref{eq:continuity_equation} is well defined in the distribution sense even when $\rho_t$ does not have a density. At each time $t$, $v_t$ can be interpreted as a tangent vector to the curve $(\rho_t)_{t\in[0,1]}$ so that the length $l((\rho_t)_{t\in[0,1]})$ of the curve $(\rho_t)_{t\in[0,1]}$ would be given by:
\begin{equation}
l((\rho_t)_{t\in[0,1]})^2 = \int_0^1 \Vert v_t \Vert^2_{L_2(\rho_t)} \dd t \quad \text{ where } \quad 
\left\Vert v_t \right\Vert^2_{L_2(\rho_t)} =  \int \left\Vert v_t(x) \right\Vert^2 \dd \rho_t(x).
\end{equation}
This perspective allows to provide a dynamical interpretation of the Wasserstein distance as the length  of the shortest path from $\nu$ to $\mu$ and is summarized by the celebrated Benamou-Brenier formula (\cite{benamou2000computational}):
\begin{align}\label{eq:benamou-brenier-formula}
W_2(\nu,\mu) = \inf_{(\rho_t,v_t)_{t\in[0,1]}} l((\rho_t)_{t\in[0,1]})
\end{align}
where the infimum is taken  over all couples  $\rho$ and $v$ satisfying  \cref{eq:continuity_equation}  with boundary conditions given by \cref{eq:boundary_conditions}. If $(\rho_t,v_t)_{t\in[0,1]}$ satisfies  \cref{eq:continuity_equation} and \cref{eq:boundary_conditions} and realizes the infimum in \cref{eq:benamou-brenier-formula}, it is then simply called a geodesic between $\nu$ and $\mu$; moreover it is called a constant-speed geodesic if, in addition, the norm of $v_t$ is constant for all $t\in[0,1]$, hence is characterized by:
\begin{equation}
    W_2(\rho_s,\rho_t)=|t-s|W_2(\rho_0,\rho_1).
\end{equation}
As a consequence, \cref{eq:displacement_geodesic} is a constant-speed displacement geodesic, and the Wasserstein space is a geodesic space \citet[Theorem 5.27]{santambrogio2015optimal}. 
Additionally, assume that $\nu$ is absolutely continuous. Then there 
 exists an optimal transport map T between $\nu$ and $\mu$; the
geodesic between $\nu$ and $\mu$ writes $\rho_t = \phi_{t\#}\nu$ where $\phi_t=((1 - t)\Id + tT)=\Id +t(T-\Id)$ and $T=\nabla \psi$ where $\psi$ is the Kantorovitch potential. In this case, $\phi_t$ is invertible and the velocity field $v_t=\nabla \psi\circ \phi_t^{-1}$.%Lemma 5.29 in Santambrogio.
\ak{comment} In the general case, the geodesics in Wasserstein space satisfy the system of coupled equations:\begin{align}    &\frac{\partial \rho_t}{\partial t}+\div(\rho_t \nabla \psi_t) = 0\\    &\label{eq:hj}\frac{\partial \psi_t}{\partial t}+ \frac{1}{2}\|\nabla \psi_t\|^2=0
\end{align}
where $\rho_0=\nu$, $v_0=\nabla \psi$. \Cref{eq:hj} is referred to as Hamilton-Jacobi equation.


\subsection{Wasserstein geometry, convexity and smoothness}


As is well-known, decay along Wasserstein gradient flows can be obtained from convexity properties along geodesics. We first define the notion of $\Lambda$-convexity.
\begin{definition}\label{def:lambda-convexity}[$\Lambda$ convexity, \cite[Definition 16.5]{villani2009optimal}]
	We say that a functional $\nu\mapsto\mathcal{F}(\nu)$ is $\Lambda$-displacement convex
	if for any constant-speed geodesic $(\rho_t,v_t)_{t \in [0,1]}$, the following holds:
\begin{equation}\label{eq:lambda_displacement_convex}
		\cF(\rho_{t})\leq(1-t)\cF(\rho_{0})+t\cF(\rho_{1})-\int_{0}^{1}\Lambda(\rho_{s},v_{s})G(s,t)ds \qquad\forall\; t\in[0,1].
	\end{equation}
	where $(\rho,v)\mapsto\Lambda(\rho,v)$ satisfies \cref{def:conditions_lambda},
	and $G(s,t)=s(1-t) \mathbb{I}\{s\leq t\}
	+t(1-s) \mathbb{I}\{s\geq t\}$ is the Green function.
	A particular case is when $\Lambda(\rho,v)= \lambda \| v\|^2_{L^2(\rho)}   $ for some $\lambda\in \R$. In that case, \cref{eq:lambda_displacement_convex} becomes:
\begin{align}\label{eq:semi-convexity}
	\cF(\rho_{t})\leq(1-t)\cF(\rho_{0})+t\cF(\rho_{1})-\frac{\lambda}{2}t(1-t)W_2^2(\rho_0,\rho_1)  \qquad\forall\; t\in[0,1].
\end{align}
In this case, $\cF$ is said to be $\lambda$-displacement convex; and in particular for $\lambda=0$, $\cF$ is said to be displacement convex.
\end{definition}

A natural object of interest is then the Hessian of the objective $\cF$. We define below this object. Recall that the tangent space of $\cP_2(\R^d)$ at $\mu \in \cP_2(\R^d)$ is defined as 
\begin{equation*}
    \mathcal{T}_{\mu}\cP_2(\R^d) = \overline{\left\{\nabla \psi, \; \psi \in \mathcal{C}_c^{\infty}(\R^d) \right\} }\subset L^2(\mu),
\end{equation*}
where the closure is taken in $L^2(\mu)$, 
see \citet[Definition 8.4.1]{ambrosio2005gradient}.

\begin{definition}\label{def:wasserstein_hessian}
The Wasserstein Hessian of a functional $\cF:\cP_2(\R^d)\to \R$ at $\mu$ is defined for any $\psi \in \mathcal{C}_c^{\infty}(\R^d)$ as:
\begin{equation*}
  \Hess_{\mu}\cF(\psi,\psi):= \dv[2]{}{t}\bigg|_{t=0} \mathcal{\cF}(\mu_t)
\end{equation*}
where $(\mu_t,v_t)_{t\in [0,1]}$ is a Wasserstein geodesic with $\mu_0=0,v_0=\nabla \psi$ (see \Cref{sec:wasserstein_geometry} for formal definitions). % = (\Id +t\nabla \psi)_{\#}\mu.
\end{definition}
\Cref{def:wasserstein_hessian} can be straightforwardly related to the usual symmetric bilinear form defined on $\mathcal{T}_{\mu}\cP_2(\R^d)\times \mathcal{T}_{\mu}\cP_2(\R^d)$ \citep[Section 3]{otto2000generalization}:
\begin{definition}
The Wasserstein Hessian of $\cF$, denoted $\Hess\cF_{|\mu}$ is an operator over $\mathcal{T}_{\mu}\mathcal{P}_2(\X)$ verifying $\ps{\Hess\cF_{|\mu}v_0, v_0}_{L^2(\mu)}=\frac{d^2}{dt^2}\Bigr|_{\substack{t=0}}\mathcal{F}(\rho_t)$ if $(\rho_t,v_t)_{t\in [0,1]}$ is a Wasserstein geodesic starting at $\mu$.
\end{definition}

Naturally, lower and upper bounds on the Hessian characterize respectively convexity and smoothness on the functional $\cF$. 
Lower bounds on the Hessian characterizes the displacement convexity of the functional, as stated in the following result from \citet[Proposition 16.2]{villani2009optimal}. 

\begin{proposition}\label{prop:villani}[\cite[Proposition 16.2]{villani2009optimal}] Let $(\rho,v)\mapsto\Lambda(\rho,v)$ an admissible functional (see \Cref{def:conditions_lambda}). 
    For any functional $\cF:\cP_2(\R^d)\to \R$, the following statements are equivalent: 
    \begin{enumerate}[label=(\roman*)]
        \item $\cF$ is $\Lambda$-displacement convex
        \item $\dv[2]{}{t}\mathcal{\cF}(\rho_t)\ge \Lambda(\rho_t,v_t)$ for a constant-speed geodesic $(\rho_t,v_t)_{t\in [0,1]}$
        \item $ \cF(\rho_1) - \cF(\rho_0)- \int \ps{\nabla \cF'(\rho_0)(x),y-x}d\pi(x,y)\ge \int_{0}^1 \Lambda(\rho_s,v_s)(1-s)ds$, where $\pi$ is an optimal coupling between $\rho_0$ and $\rho_1$ and $(\rho_t,v_t)_{t\in [0,1]}$ is a constant-speed geodesic.
    \end{enumerate}
\end{proposition}
\begin{corollary}\label{cor:convexity_characterizations}
     As a consequence of \Cref{def:lambda-convexity}, \Cref{prop:villani} and equations of Wasserstein geodesics \Cref{eq:hj}, the following statements are equivalent:
     \begin{enumerate}[label=(\roman*)]
     \item $\cF$ is $\lambda$-displacement convex
     \item $\Hess_{\mu}\cF(\psi,\psi)\ge \lambda \|\nabla \psi\|^2_{L^2(\mu)}$
     \item $ \cF(\rho_1) - \cF(\rho_0)- \int \ps{\nabla \cF'(\rho_0)(x),y-x}d\pi(x,y)\ge \frac{\lambda}{2} W_2^2(\rho_0,\rho_1)$.
     \end{enumerate}
\end{corollary}
%The proof of \Cref{prop:villani} is obtained from the equality \begin{equation}	\cF(\rho_t)=(1-t)\cF(\rho_0)+t\cF(\rho_1)-\int_{0}^{1}\dv[2]{}{s}\mathcal{\cF}(\rho_s)G(s,t)ds.\end{equation}

\begin{definition}\label{def:smooth_functional}
[Smooth functional] We will say that $\cF$ is $M$-smooth if $ \Hess_{\mu}\cF(\psi,\psi)\le M\|\nabla \psi\|^2_{L^2(\mu)} $.
\end{definition}

    \ak{to do: give other definitions of smoothness+link with lambda convexity}

\subsection{Rates for gradient descent}
We now study the Wasserstein gradient descent scheme
\begin{equation}\label{eq:wasserstein_gradient_descent}
    \mu_{l+1}=(\Id-\gamma \nabla \cF'(\mu_l))_{\#}\mu_l
\end{equation}
where $\cF'$ denotes the first variation of $\cF$ (see \Cref{def:first_variation}).

\subsubsection{Descent Lemma}
\noindent If the Hessian is upper bounded, i.e. $\cF$ is "smooth", then one can obtain a descent lemma.
\begin{proposition}\label{prop:decreasing_functional}Assume $\Hess_{\mu}\cF(\psi,\psi)\le M\|\nabla \psi\|^2_{L^2(\mu)}$ for any $\mu \in \cP_2(\R^d)$. Consider the sequence of iterates of Wasserstein gradient descent of $\cF$  defined by \eqref{eq:wasserstein_gradient_descent}. Then, the following inequality holds:
	\begin{align*}
	\cF(\mu_{l+1})-\cF(\mu_l)\leq -\gamma \left(1-\frac{\gamma}{2}M \right) \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)}.
	\end{align*}
\end{proposition}
\begin{proof}[Proof of \Cref{prop:decreasing_functional}]\label{proof:prop:decreasing_functional}
	Consider a path between $\mu_l$ and $\mu_{l+1}$ of the form $\rho_t	=(\phi_t)_{\#}\mu_l$ with $\phi_t=(\Id- t\nabla \cF'(\mu_l))$. We have $\frac{\partial \rho_t}{\partial t}= \div(\rho_t v_t)$ with $v_t=-\nabla \cF'(\mu_l)\circ \phi_t^{-1}$. The function 
 $t\mapsto\cF(\rho_t)$ is differentiable and hence absolutely continuous. Therefore one can write:
\begin{align}\label{eq:taylor_expansion_decreasing}
	\cF(\rho_{\gamma})=\cF(\rho_0) + \gamma \dv[]{}{t}\bigg|_{t=0}\cF(\rho_t)+  \int_0^{\gamma}(\gamma-t) \dv[2]{}{t}\mathcal{\cF}(\rho_t)dt.
	\end{align}
	Moreover, using the chain rule in the Wasserstein space, we have:
 \begin{equation}
    \dv[]{}{t}\cF(\rho_t) = \ps{\nabla \cF'(\rho_t), v_t}_{L^2(\rho_t)},\quad \dv[2]{}{t}\cF(\rho_t)=\ps{\Hess \cF_{|\rho_t}v_t,v_t}_{L^2(\rho_t)}
 \end{equation}
 Hence evaluating the first quantity at $t=0$ and using the transfer lemma on the second we get
 \begin{equation*}
   \dv[]{}{t}\bigg|_{t=0}\cF(\rho_t)  =-\|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)};\quad \dv[2]{}{t}\cF(\rho_t) \le M \|\nabla \cF'(\mu_l)\|^2.
 \end{equation*}
 %\tom{no $\gamma$ in the first derivative?}% yes you're right!
 Hence, the result follows directly by applying the above expressions to \Cref{eq:taylor_expansion_decreasing}.
\end{proof}

\noindent As a corollary, we obtain the convergence of the sum of squared gradients.
\begin{corollary} Let $c_{\gamma}=\gamma(1-\frac{\gamma M}{2})$. Under the assumptions of \Cref{prop:decreasing_functional}, one has
\begin{equation}
    \frac{1}{L}\sum_{l=1}^L \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)}\le \frac{\cF(\mu_0)}{2 c_{\gamma} L}.
\end{equation}
\end{corollary}
\ak{this corollary is particularly informative when the square norm of the gradient is a dissimilarity between measures (eg the Fisher divergence for the KL gradient flow, or the kernel stein discrepancy for SVGD). otherwise it's not so informative. In our case since the functional $\cF_{\epsilon}$ is the KL, we obtain the Fisher divergence:
\begin{equation*}
    \|\nabla \cF_{\epsilon}'(\mu)\|^2_{L^2(\mu)}= \left\Vert\nabla \log\left(\frac{\ke\star\mu}{\tg}\right)\right\Vert^2_{L^2(\ke\star\mu)}
\end{equation*}}


%\subsubsection{Rates under a functional inequality}


\subsubsection{Rates for Lamda-convex functionals}

\noindent Additionally, if the functional is $\Lambda$-displacement convex, one can obtain rates of convergence in terms of the objective $\cF$.
\begin{theorem}\label{th:rates_convex} Assume that $\cF$ is $M$-smooth. Moreover, assume that $\cF$ is $\Lambda$--convex. 
	Let $\bar{K}_l$ be the average of $(K(\mu_j))_{0\leq j \leq l}$ where $(\rho^j_t)_{0\leq t \leq 1}$ is a constant-speed geodesic from $\mu_j$ to $\tg$ and $K(\mu_j):=\int_0^1 \Lambda(\rho^j_s,v^j_s)(1-s)ds$, where $\mu_j$ is defined by \eqref{eq:wasserstein_gradient_descent}. Then, the following inequality holds for any $l\ge0$:
\begin{align}
\cF(\mu_l) \leq  \frac{W_2^2(\mu_0,\tg)}{2 \gamma l} -\bar{K}_l.
\end{align}
\end{theorem}
\Cref{th:rates_convex} is obtained using techniques from optimal transport and optimization. It relies on $\Lambda$-convexity and a descent lemma to prove an \textit{extended variational inequality}, and concludes using a suitable Lyapunov function. A full proof is given in \Cref{sec:descent_barrier}.
When $\bar{K}$ is non-negative, one recovers the usual convergence rate as $O(\frac{1}{l})$ for the gradient descent algorithm. However, $\bar{K}$ can be negative in general, and would therefore act as a barrier on the optimal value that $\cF(\mu_l)$ can achieve when $l\rightarrow \infty$. \\

\noindent In particular, when $\Lambda(\rho,v)= \lambda \| v\|^2_{L^2(\rho)}   $, we can get a more explicit expression as stated in the following corollary.

\begin{corollary}\label{cor:rates}
    Suppose that the assumptions of \Cref{th:rates_convex} hold and that 
    $\Lambda(\rho,v)=\lambda \|v\|^2_{L^2(\rho)}.$ Then for any $l\ge 0$:
    \begin{align}\label{eq:rate_gd}
\cF(\mu_l) \leq  \frac{W_2^2(\mu_0,\tg)}{2 \gamma l} -\frac{\lambda}{l}\sum_{j=0}^l W_2^2(\mu_j,\tg).
\end{align}
\end{corollary}
Once again, if $\lambda$ is negative, the second term on the right hand side of \eqref{eq:rate_gd} acts as a barrier.\\
 \ak{GOAL: get an upper and lower bound on the Hessian of the regularized relative entropy $\cF_{\epsilon}$; to get convergence rates for gradient descent with an explicit value of the $\lambda$-convexity constant with respect to $\epsilon$. }



\subsubsection{Proof of  \Cref{th:rates_convex}}\label{sec:descent_barrier}

To provide a proof of \Cref{th:rates_convex}, we need the following preliminary results. Firstly, an upper-bound on a scalar product involving $\nabla \cF'(\mu)$ for any $\mu \in \mathcal{P}_2(\X)$ in terms of the loss functional $\cF$, is used from the $\Lambda$-displacement convexity of $\cF$, see \Cref{prop:villani}. Then, an EVI (Evolution Variational Inequality) is obtained in on the gradient flow of $\cF$ using as well the descent lemma \Cref{prop:decreasing_functional}. Finally, a suitable Lyapunov function is used to obtained the rates of convergence.



\begin{proof}
	Let $\pi^l$ be the optimal coupling between $\mu_l$ and $\tg$, then the optimal transport between $\mu_l$ and $\mu$ is given by:
	\begin{align}
	W_2^2(\mu_l,\tg)=\int \Vert x-y \Vert^2 d\pi^l(x,y)
	\end{align}
	Moreover, consider $z=x-\gamma \nabla \cF'(\mu_l)(x)$ where $(X,Y)\sim \pi^l$. Then $(Z,Y)$ is a coupling between $\mu_{l+1}$ and $\tg$, therefore, by definition of the Wasserstein distance it follows that:
	\begin{align}\label{eq:optimal_upper-bound}
	W_2^2(\mu_{l+1},\tg)\leq \int \Vert x-\gamma \nabla \cF'(\mu_l)(x)-y\Vert^2 d\pi^l(x,y)
	\end{align}
	By expanding the r.h.s in \cref{eq:optimal_upper-bound}, the following inequality holds:
	\begin{align}\label{eq:main_inequality}
	W_2^2(\mu_{l+1},\tg)\leq W_2^2(\mu_{l},\tg) -2\gamma \int \langle \nabla \cF'(\mu_l)(x), x-y \rangle d\pi^l(x,y)+ \gamma^2 \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)}.
	\end{align}
	Since $\cF$ is $\Lambda$-convex, by \Cref{prop:villani} it holds that:
	\begin{align}\label{eq:flow_upper-bound}
	-2\gamma \int   \ps{\nabla\cF'(\mu_l)(x),x-y} d\pi^l(x,y)
	\leq
	-2\gamma\left(\cF(\mu_l)- \cF(\tg) +K(\mu^l)\right)
	\end{align}
	where $(\rho^l_t)_{0\leq t \leq 1}$ is a constant-speed geodesic from $\mu_l$ to $\tg$ and $K(\mu^l):=\int_0^1 \Lambda(\rho^l_s,v^l_s)(1-s)ds$. 
	Note that when $K(\mu^l)\leq 0$ it falls back to the convex setting.
	Therefore, the following inequality holds:
	\begin{align}
	W_2^2(\mu_{l+1},\tg)\leq W_2^2(\mu_{l},\tg) - 2\gamma\left(\cF(\mu_l)- \cF(\tg) +K(\mu^l)\right) +\gamma^2 \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)}.
	\end{align}
	Now we introduce a term involving $\cF(\mu_{l+1})$. The above inequality becomes:
	\begin{align}
	W_2^2(\mu_{l+1},\tg)\leq & W_2^2(\mu_{l},\tg) - 2\gamma\left(\cF(\mu_{l+1})- \cF(\tg) +K(\mu^l)\right) \\
	&+\gamma^2  \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)} -2\gamma (\cF(\mu_l)-\cF(\mu_{l+1}))
	\label{eq:main_ineq_2}
	\end{align}
	The last two terms on the r.h.s. of the previous inequality are upper bounded when the step-size is small enough by \Cref{prop:decreasing_functional}:
	\begin{align}
	\gamma^2 \|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)} -2\gamma (\cF(\mu_l)-\cF(\mu_{l+1})\leq -\gamma^2 (1-\frac{\gamma M}{2})\|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)},
	\label{eq:decreasing_functional}
	\end{align}
	where $M$ is the smoothness constant of $\cF$. Combining  \cref{eq:main_ineq_2} and \cref{eq:decreasing_functional} we obtain:
	\begin{align}
	2\gamma(\cF(\mu_{l+1})-\cF(\tg))+\gamma^2(1-\frac{\gamma M}{2})\|\nabla \cF'(\mu_l)\|^2_{L^2(\mu_l)}
	\leq 
	W_2^2(\mu_l,\tg)-W_2^2(\mu_{l+1},\tg)-2\gamma K(\mu^l).
	\label{eq:main_final}
	\end{align}
	and for $\gamma \le 1/2M$ we finally obtain  the following \textit{evolution variational inequality} (EVI):
 	\begin{align}
	2\gamma(\cF(\mu_{l+1})-\cF(\tg))
	\leq 
	W_2^2(\mu_l,\tg)-W_2^2(\mu_{l+1},\tg)-2\gamma K(\mu^l).
	\label{eq:evi_final}
	\end{align}
Now, consider the Lyapunov function $L_j = j \gamma (\cF(\mu_l) - \cF(\tg)) + \frac12 W_2^2(\mu_j,\mu)$ for any iteration $j$. At iteration $j+1$, we have:
	\begin{align*}
	L_{j+1} &= j\gamma(\cF(\mu_{j+1}) - \cF(\tg)) + \gamma(\cF(\mu_{j+1}) - \cF(\tg)) + \frac12 W_2^2(\mu_{j+1},\tg)\\
	&\leq j\gamma(\cF(\mu_{j+1}) - \cF(\mu)) + \frac12 W_2^2(\mu_j,\tg)-\gamma K(\mu^j)\\
	&\leq j\gamma(\cF(\mu_{j}) - \cF(\tg)) + \frac12 W_2^2(\mu_j,\tg)-\gamma K(\mu^j) -j\gamma^2 (1-\frac{\gamma M}{2} )\|\nabla \cF(\mu_j)\|^2_{L^2(\mu_j)} \\
	&\leq  L_j - \gamma K(\mu^j).
	\end{align*}
	where we used the EVI \eqref{eq:evi_final} and \Cref{prop:decreasing_functional} successively for the two first inequalities. We thus get by telescopic summation: 
	\begin{equation}
	 L_l \leq L_0 -\gamma \sum_{j = 0}^{l-1} K(\mu^j)
	\end{equation}
		Let us denote $\bar{K}$ the average value of $(K(\mu^l))_{0\leq j \leq l}$ over iterations up to $l$. We can now write the final result:
	\begin{equation}
	\cF(\mu_{l}) - \cF(\tg) \leq \frac{W_2^2(\mu_0, \tg)}{2 \gamma l} -\bar{K}.\qedhere
	\end{equation}
\end{proof}


